RoRA-VLM: Robust Retrieval-Augmented Vision Language Models

Current vision-language models (VLMs) still exhibit inferior performance on knowledge-intensive tasks, primarily due to the challenge of accurately encoding all the associations between visual objects and scenes to their corresponding entities and background knowledge. While retrieval augmentation methods offer an efficient way to integrate external knowledge, extending them to vision-language domain presents unique challenges in (1) precisely retrieving relevant information from external sources due to the inherent discrepancy within the multimodal queries, and (2) being resilient to the irrelevant, extraneous and noisy information contained in the retrieved multimodal knowledge snippets. In this work, we introduce RORA-VLM, a novel and robust retrieval augmentation framework specifically tailored for VLMs, with two key innovations: (1) a 2-stage retrieval process with image-anchored textual-query expansion to synergistically combine the visual and textual information in the query and retrieve the most relevant multimodal knowledge snippets; and (2) a robust retrieval augmentation method that strengthens the resilience of VLMs against irrelevant information in the retrieved multimodal knowledge by injecting adversarial noises into the retrieval-augmented training process, and filters out extraneous visual information, such as unrelated entities presented in images, via a query-oriented visual token refinement strategy. We conduct extensive experiments to validate the effectiveness and robustness of our proposed methods on three widely adopted benchmark datasets. Our results demonstrate that with a minimal amount of training instance, RORA-VLM enables the base model to achieve significant performance improvement and constantly outperform state-of-the-art retrieval-augmented VLMs on all benchmarks while also exhibiting a novel zero-shot domain transfer capability.

==> body/2_method_old.tex <==
% \section{Method}

\section{\alignment{}}
% motivation
Prior research~\cite{KeyValueGeva2021, locateFactMeng2022} identifies that the knowledge of large language models (LLMs) mainly resides in their feedforward multi-layer perceptrons (MLPs). The first layers $\mathbf{W}_{up}$ in MLPs store the the keys correlated with input text-pattern and the memory coefficients computed from the key matrix and input decide the vocabulary distribution of the next token. We adopt this key–value memory perspective and propose to intervene the internal knowledge retrieving process with visual features.
% from \cite{KeyValueGeva2021} which hypothesizes that the first layers $\mathbf{W}_{up}$ in MLPs store the the keys correlated with text-pattern and the key values are associated with output distributions over vocabularies.
% Inspired by this finding, we propose a novel architecture, vision-knowledge alignment (\arch{}), designed to bridge the gap between textual entity knowledge and visual image information.
% what it is
Unlike traditional vision language models (VLMs) that separately process and then concatenate text and image features before input into LLMs~\cite{}, \arch{} introduces an innovative integration strategy to enhance the interaction between visual and textual modalities. It incorporates an additional projector layer and an gate layer within each decoder block of the transformer architecture.  The raw image features, encoded by the CLIP model~\cite{}, are projected into the latent space of the LLM via the new projector layer and then are independently fed into the newly added gate layer. This gate projection layer adjusts the activation function biases based on the visual input and adds those biases to the standard MLP layer within a transformer decoder block. The combined activation biases are subsequently processed through the standard up and down projection layers, maintaining the workflow of the traditional transformer decoders. 

% how to do it
Specifically, for a given text query $\mathbf{Q}$ and an image $\mathbf{I}$, we firstly use a pre-trained CLIP visual encoder to extract visual features $\mathbf{Z}_I=g(\mathbf{I})$ and its [CLS] token representation $\mathbf{z}_{cls}=\mathbf{Z}_I[:,:1,:]$. The visual features $\mathbf{Z}_I=g(\mathbf{I})$ is converted into the latent space of the language model by a projection matrix $\mathbf{W}$, resulting in $\mathbf{H}_I$. This embedding is then concatenated with the query embedding $\mathbf{H}_Q$ to form a unified input sequence $\mathbf{H}=[\mathbf{H}_I,\mathbf{H}_Q]$. To align the visual feature with the textual understanding of LLMs, we introduce a bias adjustment directly into the MLP layers of the language model. This is achieved by employing two trainable projection matrices, $\mathbf{W}_p$ and $\mathbf{W}_g$, across the decoder layers. $\mathbf{W}_p$ adapts $\mathbf{z}_{cls}$ into an embedding vector $\mathbf{h}_{cls}$ that matches the latent dimensions of the language model. To uniformly influence the representation of each token, $\mathbf{h}_{cls}$ is replicated into a sequence $\mathbf{H}_{cls}$ that matches the length $n_H$ of $\mathbf{H}$. Further, we use $\mathbf{W}_g$ to simulate a gate projection to stimulate the activation function and then to generate the bias. Consequently, the modified MLP layer operation can be articulated as follows:
% \jy{equation: long single line / short multiple lines}
% \begin{equation}
%     \text{MLP}(\mathbf{H}, \mathbf{H}_{cls}) = \text{ReLU}(\mathbf{W}_{dw} \cdot \left( w_1 \cdot \phi(\mathbf{W}_{g1} \cdot \mathbf{H} + \mathbf{b}_{g1}) + w_2 \cdot \phi(\mathbf{W}_{g2} \cdot \mathbf{H}_{cls} + \mathbf{b}_{g2}) \right) \odot (\mathbf{W}_{up} \cdot \mathbf{H} + \mathbf{b}_{up}) + \mathbf{b}_{dw}) \\
% \end{equation}
\begin{equation}
\begin{split}
    \text{MLP}(\mathbf{H}, \mathbf{H}_{cls}) &= \text{ReLU}(\text{down\_proj}(\mathbf{a}\odot \text{up\_proj}(\mathbf{H}))) \\
    \mathbf{a} &= w_1 \cdot \phi(\text{gate\_proj}(\mathbf{H})) + w_2 \cdot \phi(\text{gate\_proj2}(\mathbf{H}_{cls})) \\
    \mathbf{H_{cls}} &= n_H\times[\mathbf{h}_{cls}]\text{, with }\mathbf{h}_{cls} = \mathbf{W}_p \cdot \mathbf{z_{cls}} = \mathbf{W}_p \cdot \mathbf{Z}_I[:,:1,:]
\end{split}
\end{equation}
with
\begin{equation}
    \begin{split}
        & \text{up\_proj}(\mathbf{x}) = \mathbf{W}_{up} \cdot \mathbf{x} + \mathbf{b}_{up} \\
        & \text{down\_proj}(\mathbf{x}) = \mathbf{W}_{dw} \cdot \mathbf{x} + \mathbf{b}_{dw} \\
        & \text{gate\_proj}(\mathbf{x}) = \mathbf{W}_{g_{std}} \cdot \mathbf{x} + \mathbf{b}_{g_{std}} \\
        & \text{gate\_proj'}(\mathbf{x}) = \mathbf{W}_{g} \cdot \mathbf{x} + \mathbf{b}_{g}  
    \end{split}
\end{equation}
% where $\mathbf{W}_{up}$, $\mathbf{W}_{dw}$, $\mathbf{W}_{g}$, $\mathbf{W}_{g_{std}}$, and $\mathbf{W}_{p}$ are trainable matrices. $w_1$ and $w_2$ are trainable weights constrained by $\sum(w_1, w_2)=1$.
where $\mathbf{W}_{up}$ and $\mathbf{W}_{dw}$ are trainable matrices responsible for the up and down projections within the MLP layer, respectively. $\mathbf{W}_{g}$ and $\mathbf{W}_{g_{std}}$ denote the trainable gating matrices that modulate the flow of information based on the visual and textual inputs. $\mathbf{W}_{p}$ is the projection matrix that aligns the visual feature representation with the language model's latent space. The weights $w_1$ and $w_2$ are trainable parameters, optimized subject to the constraint $\sum(w_1, w_2)=1$, ensuring a normalized combination of features from different modalities. 




% summary
\section{Retrieval Augmented Generation}
To bridge the knowledge gap for entities unseen during training, we enhance our model's capability by integrating a Retrieval Augmented Generation (RAG) framework. Given an input image $\mathbf{I}$, our model retrieves relevant multimodal documents $\mathbf{R}$, leveraging them as supplementary context in the generation of output $\mathbf{y}$. This framework involves two core components: (i) an image-based retriever $p_r(\mathbf{R}|\mathbf{I})$, designed to fetch a list of image-text pair passages in response to a given query image $\mathbf{I}$, and (ii) a multimodal interleave generator $p_g(y_i|\mathbf{R}, \mathbf{I},\mathbf{T},y_{1:{i-1}})$, responsible for generating the next token $y_i$ by integrating the preceding tokens $y_{1:{i-1}}$, original input query $\mathbf{T}$, input image $\mathbf{I}$, and retrieved multimodal documents $\mathbf{R}$.

\subsubsection{Robust Vision Language Retrieval}
% motivation
We developed an image-based entity retriever to enhance the background knowledge extraction for entities in images. This retriever uses the image feature to identify and retrieve additional information about entities, thereby augmenting our model's ability to handle previously unseen entities.

% what it is and how to do it
For an input query image $\mathbf{I}$, the goal of our retriever is to identify and retrieve the top $k$ images that involve the same entity, along with their associated textual data. To build our retriever, we utilize the Wikipedia-based image-text dataset (WIT)~\cite{}, which comprises over 11.4 million unique images. For each image, we collect up to three textual contexts: image caption, section title, and section text, where available. Then, we employ an image encoder model to extract feature vectors from images. Specifically, each image in the WIT dataset is processed through CLIP~\cite{} to generate a corresponding image feature vector. These vectors are then organized into a Hierarchical Navigable Small World (HNSW) graph, facilitating efficient nearest neighbor searches.

Upon receiving a query image $\mathbf{I}$, we extract its image feature vector using the CLIP model. This vector serves as the query to retrieve the $k$ nearest feature vectors in the HNSW graph, searching images that likely represent the same entity. 
% \begin{equation}
%     p_n(z|x) \propto \text{exp} (\mathbf{d}(z)^\mathrm{T}\mathbf{q}(x))\text{, }\mathbf{d}(z)=\text{BERT}_d(z)\text{, }\mathbf{q}(x)=\text{BERT}_q(x)
% \end{equation}
\begin{equation}
    p_k(\mathbf{R}|\mathbf{I}) \propto \text{HNSW} (\mathbf{d}(\mathbf{R}_i)^\top \mathbf{q}(\mathbf{I}))\text{, }\mathbf{d}(\mathbf{R}_i)=\text{CLIP}(\mathbf{R}_i)\text{, }\mathbf{q}(\mathbf{I})=\text{CLIP}(\mathbf{I})
\end{equation}

For each retrieved image, we extract and return the following information, forming a list $\mathbf{R} = \{\mathbf{r}_1, \ldots, \mathbf{r}_k\}$ where each $\mathbf{r}_i$ is a tuple containing:

\begin{itemize}
    \item IMG: an image that contains same entity as the query image,
    \item IMG\_CAP: the image caption,
    \item SEC\_TITLE: the title of the section in which the image is used,
    \item SEC\_TEXT: the text of the section associated with the image.
\end{itemize}

\subsubsection{Interleave Multimodality Input}
To effectively integrate the inputs $\mathbf{T}$, $\mathbf{I}$, and the retrieved multimodal content $\mathbf{R}$ into a uniform input sequence for our VLM, we concatenate them together. Given the constraints on input length imposed by our language model, we employ a pooling strategy on both the retrieved images within $\mathbf{R}$ and the input image $\mathbf{I}$ to manage their spatial dimensions efficiently.
\paragraph{Pooling}
After extracting image features $\mathbf{Z}$ using the vision tower of the CLIP model, we apply a structured pooling operation to reduce the spatial dimensions of these features to fit the model’s input constraints while preserving essential spatial information. The initial image features extracted via the vision tower of the CLIP model result in a three-dimensional tensor of shape $(b, n, c)$ where $b$ represents the batch size, $n$ is the number of features, and $c$ is the channel dimension. To facilitate a structured reduction of this feature map, we first reshape the tensor into a square format $(b, c, \sqrt{n}, \sqrt{n})$, aligning with the spatial dimensions of the image. Subsequently, we implement an average pooling operation:
\begin{equation}
    \mathbf{Z}' = \text{pool2d}(\mathbf{Z}_{\text{reshaped}}, \text{kernel size} = (s, s), \text{stride} = s)
\end{equation}
where $s = \frac{\sqrt{n}}{\sqrt{64}}$ denotes the stride and kernel size, calculated by the square root of the initial feature count divided by the square root of the desired feature coun. In this work, we use 64 as the desired feature coun.

Moreover, we implement a truncation procedure for the text passages retrieved in $\mathbf{R}$, adapting their length to comply with the input size limits of our language model. This truncation process prevents the exclusion of subsequent passages by maintaining only the initial segment of the text, ensuring diverse content integration. Finally, the multimodal interleave generation process can be formally described as:
\begin{equation}
\begin{split}
    p_g(y_i|\mathbf{R',\mathbf{I}}, \mathbf{T},y_{1:{i-1}}) 
    &= p_g(y_i|\mathbf{r}_1^I, \mathbf{r}_1^T,...,\mathbf{r}_k^I, \mathbf{r}_k^T,\mathbf{I},\mathbf{T},y_{1:{i-1}}) \\
    &= p_g(y_i|\mathbf{Z}'_1, \mathbf{r}_1^T,...,\mathbf{Z}'_k, \mathbf{r}_k^T,\mathbf{Z}'_I,\mathbf{T},y_{1:{i-1}})
\end{split}
\end{equation}

==> body/2_method_old2.tex <==
\section{\arch{}: Synergistic Knowledge Alignment and Augmentation}
In this section, we first explain our base VLM and \alignment{} pre-training. Then, we recap the retrieval augmented generation in the text-only setting and introduce our \retrieval{} method.  
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{imgs/overview.pdf}
    \caption{\jy{todo: caption}}
    \label{fig:overview}
\end{figure*}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{imgs/overview2.pdf}
    \caption{\jy{todo: caption}}
    \label{fig:overview}
\end{figure*}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{imgs/overview3.pdf}
    \caption{\jy{todo: caption}}
    \label{fig:overview}
\end{figure*}

\subsection{\alignment{}}

\paragraph{Base VLM} We adopt the pretrained LLaVA 1.5~\cite{llava1.5} as our base VLM due to its strong performance. LLaVA consists of a pretrained CLIP image encoder, a pretrained LLM to generate text, and a MLP projector to map visual features into the LLM's semantic space. LLaVA is pretrained on large-scale image-caption pairs. During pretraining the  CLIP encoder and the LLM remain frozen and only the MLP projector is trained. Formally, given an image $I$ and a text query $q$, the CLIP encoder encodes the image into a sequence of image-patch vectors $\mathbf{X}_{I}\in\mathbb{R}^{s\times d}$ and a image concept vector $\mathbf{x}_{cls}\in\mathbb{R}^{d}$ where $s$ is the number of encoded image patches and $d$ is the hidden dimension of CLIP. The MLP projector $f_{\text{pro}}:\mathbb{R}^{d}\rightarrow\mathbb{R}^D$ maps the sequence of image vectors into the semantic space of the LLM, $\mathbf{H}_{I}=f_{\text{pro}}(\mathbf{X}_{I})\in \mathbb{R}^{s\times D}$ where $D$ is the LLM's hidden dimension. The text query passes through the embedding layer of the LLM and becomes the initial hidden representations $\mathbf{H}_q\in\mathbb{R}^{S\times D}$, where $S$ is the length of the query. The mapped image representations are concatenated to query hidden representations to form $\mathbf{H}=[\mathbf{H}_{I}:\mathbf{H}_{q}]$ and $\mathbf{H}$ is fed into transformer blocks.

\paragraph{Knowledge-intensive Pretraining Improves Robustness}
\jy{todo}

\subsection{\retrieval{}}

REALMs~\cite{rag,realm} often consist of a retriever, an external knowledge source, and a generator. Given a text query $q$,   the retriever fetches a set of documents $\mathbf{R} = \{\mathbf{r}_1, \mathbf{r}_2, \ldots, \mathbf{r}_k\}$ that are most relevant to $q$ from the external knowledge source. The generator, typically a LLM, uses these retrieved documents as additional context to generate the output sequence $\mathbf{y}$ conditioned on the text query $q$:
\begin{equation}
p_g(\mathbf{y}|q, \mathbf{R}) = \prod_{i=1}^{n} p_g(y_i|q, \mathbf{R}, y_{1:i-1})
\end{equation}
where $p_g$ represents the probability distribution over sequences of tokens defined by the LLM and $y_i$ is the $i$-th token of the output sequence.

\subsubsection{Vision-Language Retrieval}
In this part, we explain how to extend the text-only retrieval to fit the vision-language setting. We develop a two-stage vision-language retrieval to explore entity information from external knowledge sources. 

\paragraph{Image Retriever}
The first stage is a query-independent image retriever. We leverage WIT~\cite{} as the external knowledge source in this work, which consists of 37.6 million entity-rich image-text pairs. Each text is a knowledge snippet crawled from Wikipedia pages containing the captions and background knowledge of the entities in the image.
We use CLIP encoder to encode all images in WIT into search index $\mathbf{Z}=\{\mathbf{z}_1,\mathbf{z}_2,...,\mathbf{z}_N\}$ and entity names are search values $\mathbf{E}=\{e_1,e_2,...,e_N\}$, where $N$ denote the total number of entries in WIT. The retriever $f^{\text{img}}_{\text{re}}$ leverages a non-parametric function to measure cosine-similarity between two image vectors. The similarity measurement function can be expressed as:
\begin{equation}
p_r(\mathbf{I}_{\text{re}}|I) \propto \text{HNSW}(\mathbf{d}(\mathbf{Z})^\top \mathbf{q}(I))
\end{equation}
where $\mathbf{I}_{\text{re}}=\{I_1, I_2,...,I_k\}$ denotes the retrieved images. Based on this function, given an image $I$ and a text query $q$, the retriever fetches the top-k images that are most similar to the query image together with their Wikipedia knowledge.
\begin{equation}
\{(I_1,e_1),(I_2,e_2),...,(I_k,e_k)\}=f_{\text{re}}(I,\mathbf{Z}, \mathbf{E})
\end{equation}
where $I_i$ denotes the $\textit{i}$-th retrieved image and and $e_i$ denotes its entity name. 

\paragraph{Text Retriever}
With the entity name of each retrieved image, we develop the second stage text-retriever with an online serper. Given a text query \textit{q} and with a potential entity name \textit{e}, the retriever $f^{\text{txt}}_{\text{re}}$ searches the external knowledge snippets $c$ that are most relevant to the query. 
\begin{equation}
\{c_1, c_2,...,c_k\}=f^{\text{txt}}_{\text{re}}(q,\mathbf{I}_{\text{re}})
\end{equation}
where $c_i$ denotes the corresponding external knowledge snippet to the entity involved in $\textit{i}$-th retrieved image. 

Finally, the retrieved passages for generation augmentation can be denote as:
\begin{equation}
    \mathbf{R} = \{\mathbf{r}_1, \mathbf{r}_2, \ldots, \mathbf{r}_k\}=\{(I_1,c_1),(I_2,c_2),...,(I_k,c_k)\}
\end{equation}

\subsubsection{Multimodality Interleaved Generation}
These retrieved multimodal documents are interleaved and used as additional context for generating the output sequence. We concatenate the input query and interleaved documents into a uniform sequence as input for our VLM. We prepend the the retrievals to $(I,q)$ and form the interleaved input sequence $\mathbf{X}=[I_1,c_1,I_2,c_2,...,I_k,c_k,I,q]$. We input $\mathbf{X}$ into the VLM (generator) to generate the response $\mathbf{y}$.

\paragraph{Mixture of Passages Training}
In addition, our goal is to teach VLMs to be robust to irrelevant entity images and corresponding contexts. We design to intensively import irrelevant retrieved passages as noise into the training instances to force the model to learn the capability of determination. To create training examples with both relevant/irrelevant contexts, we return the top-2 retrieved images and corresponding knowledge snippets $\{(I_1,c_1),(I_2,c_2)\}$ and randomly fetch a retrieved image and context $(I'_1,c'_1)$ for another query $\{\textit{I'}, \textit{q'}\}$. The training dataset is defined by $D=\{([I_1,c_1,I_2,c_2,I'_1,c'_1;I,q],a)\}$.

\paragraph{Vision Patch Selection}
Given the constraints on input length imposed by our language model, we employ a visual token selection strategy on both the retrieved images $\mathbf{I}_{\text{re}}$ and the query image $I$ to manage their spatial dimensions efficiently. Given an image $I$ and a text query $q$, the CLIP encoder encodes the image into a sequence of image-patch vectors $\mathbf{X}_{I}\in\mathbb{R}^{s\times d}$, where $s$ is the number of encoded image patches. Intuitively, the significance of each patch is different for different queries. Due to the limited input length, we hope the models could focus on patches that are more relevant to the query instead of equal attention to all patches. So, we also encode the test query $q$ with the same CLIP encoder into a sequence of text vector $\mathbf{X}_{q}\in\mathbb{R}^{s'\times d}$, where $s'$ is the number of text tokens. For each image patch vector $\mathbf{x}^I_i\in\mathbb{R}^{d}$, we calculate the similarity (i.e., distance between vector in the latent space) to all text tokens $\text{s}_i=\sum^{s'}_{j=1}\mathbf{x}^I_i \otimes \mathbf{x}^q_j$, and fetch the top-l most relevant image-patch vectors. The final image-patch vectors $\mathbf{X}_{I'}\in\mathbb{R}^{l\times d}$ is:
\begin{equation}
    \mathbf{X}_{I'} = \text{Top-}l \left( \left\{\mathbf{x}^I_i \, \bigg| \, \sum_{j=1}^{s'} \mathbf{x}^I_i \cdot \mathbf{x}^q_j \right\}_{i=1}^{s} \right)
\end{equation}
In this work, we use $l$ = 64 as the desired feature count.



Given the constraints on input length imposed by our language model, we employ a dimension reduction strategy on both the retrieved images $\mathbf{I}_{\text{re}}$ and the query image $I$ to manage their spatial dimensions efficiently.
The most straightforward way is average pooling. We apply a structured pooling operation to reduce the spatial dimensions of image features $\mathbf{Z}$ to fit the model’s input constraints while preserving essential spatial information. The initial image features extracted via the vision tower of the CLIP model result in a three-dimensional tensor of shape $(b, n, c)$ where $b$ represents the batch size, $n$ is the number of features, and $c$ is the channel dimension. To facilitate a structured reduction of this feature map, we first reshape the tensor into a square format $(b, c, \sqrt{n}, \sqrt{n})$, aligning with the spatial dimensions of the image. Subsequently, we implement an average pooling operation:
\begin{equation}
    \mathbf{Z}' = \text{pool2d}(\mathbf{Z}_{\text{reshaped}}, \text{kernel size} = (s, s), \text{stride} = s)
\end{equation}
where $s = \frac{\sqrt{n}}{\sqrt{64}}$ denotes the stride and kernel size, calculated by the square root of the initial feature count divided by the square root of the desired feature count. In this work, we use 64 as the desired feature count.\jy{TODO HERE}




==> custom <==
@inproceedings{locateFactMeng2022,
  author       = {Kevin Meng and
                  David Bau and
                  Alex Andonian and
                  Yonatan Belinkov},
  editor       = {Sanmi Koyejo and
                  S. Mohamed and
                  A. Agarwal and
                  Danielle Belgrave and
                  K. Cho and
                  A. Oh},
  title        = {Locating and Editing Factual Associations in {GPT}},
  booktitle    = {Advances in Neural Information Processing Systems 35: Annual Conference
                  on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans,
                  LA, USA, November 28 - December 9, 2022},
  year         = {2022},
  url          = {http://papers.nips.cc/paper\_files/paper/2022/hash/6f1d43d5a82a37e89b0665b33bf3a182-Abstract-Conference.html},
  timestamp    = {Mon, 08 Jan 2024 16:31:36 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/MengBAB22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{dai2024nvlm,
  title={NVLM: Open Frontier-Class Multimodal LLMs},
  author={Dai, Wenliang and Lee, Nayeon and Wang, Boxin and Yang, Zhuoling and Liu, Zihan and Barker, Jon and Rintamaki, Tuomas and Shoeybi, Mohammad and Catanzaro, Bryan and Ping, Wei},
  journal={arXiv preprint arXiv:2409.11402},
  year={2024}
}

@inproceedings{wikillava,
  title={Wiki-LLaVA: Hierarchical Retrieval-Augmented Generation for Multimodal LLMs},
  author={Caffagni, Davide and Cocchi, Federico and Moratelli, Nicholas and Sarto, Sara and Cornia, Marcella and Baraldi, Lorenzo and Cucchiara, Rita},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1818--1826},
  year={2024}
}

@inproceedings{KeyValueGeva2021,
  author       = {Mor Geva and
                  Roei Schuster and
                  Jonathan Berant and
                  Omer Levy},
  editor       = {Marie{-}Francine Moens and
                  Xuanjing Huang and
                  Lucia Specia and
                  Scott Wen{-}tau Yih},
  title        = {Transformer Feed-Forward Layers Are Key-Value Memories},
  booktitle    = {Proceedings of the 2021 Conference on Empirical Methods in Natural
                  Language Processing, {EMNLP} 2021, Virtual Event / Punta Cana, Dominican
                  Republic, 7-11 November, 2021},
  pages        = {5484--5495},
  publisher    = {Association for Computational Linguistics},
  year         = {2021},
  url          = {https://doi.org/10.18653/v1/2021.emnlp-main.446},
  doi          = {10.18653/V1/2021.EMNLP-MAIN.446},
  timestamp    = {Fri, 16 Feb 2024 08:27:36 +0100},
  biburl       = {https://dblp.org/rec/conf/emnlp/GevaSBL21.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{encyclopedic,
  author       = {Thomas Mensink and
                  Jasper R. R. Uijlings and
                  Llu{\'{\i}}s Castrej{\'{o}}n and
                  Arushi Goel and
                  Felipe Cadar and
                  Howard Zhou and
                  Fei Sha and
                  Andr{\'{e}} Ara{\'{u}}jo and
                  Vittorio Ferrari},
  title        = {Encyclopedic {VQA:} Visual questions about detailed properties of
                  fine-grained categories},
  booktitle    = {{IEEE/CVF} International Conference on Computer Vision, {ICCV} 2023,
                  Paris, France, October 1-6, 2023},
  pages        = {3090--3101},
  publisher    = {{IEEE}},
  year         = {2023},
  url          = {https://doi.org/10.1109/ICCV51070.2023.00289},
  doi          = {10.1109/ICCV51070.2023.00289},
  timestamp    = {Tue, 07 May 2024 20:06:55 +0200},
  biburl       = {https://dblp.org/rec/conf/iccv/MensinkUCGCZSAF23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{infoseek,
    title = "Can Pre-trained Vision and Language Models Answer Visual Information-Seeking Questions?",
    author = "Chen, Yang  and
      Hu, Hexiang  and
      Luan, Yi  and
      Sun, Haitian  and
      Changpinyo, Soravit  and
      Ritter, Alan  and
      Chang, Ming-Wei",
    editor = "Bouamor, Houda  and
      Pino, Juan  and
      Bali, Kalika",
    booktitle = "Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing",
    month = dec,
    year = "2023",
    address = "Singapore",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2023.emnlp-main.925",
    doi = "10.18653/v1/2023.emnlp-main.925",
    pages = "14948--14968",
    abstract = "Pre-trained vision and language models have demonstrated state-of-the-art capabilities over existing tasks involving images and texts, including visual question answering. However, it remains unclear whether these models possess the capability to answer questions that are not only querying visual content but knowledge-intensive and information-seeking. In this study, we introduce InfoSeek, a visual question answering dataset tailored for information-seeking questions that cannot be answered with only common sense knowledge. Using InfoSeek, we analyze various pre-trained visual question answering models and gain insights into their characteristics. Our findings reveal that state-of-the-art pre-trained multi-modal models (e.g., PaLI-X, BLIP2, InstructBLIP) face challenges in answering visual information-seeking questions, but fine-tuning on the InfoSeek dataset elicits models to use fine-grained knowledge that was learned during pre-training. Furthermore, we show that accurate visual entity recognition can be used to improve performance on InfoSeek by retrieving relevant documents, showing a significant space for improvement.",
}

@inproceedings{oven,
  author       = {Hexiang Hu and
                  Yi Luan and
                  Yang Chen and
                  Urvashi Khandelwal and
                  Mandar Joshi and
                  Kenton Lee and
                  Kristina Toutanova and
                  Ming{-}Wei Chang},
  title        = {Open-domain Visual Entity Recognition: Towards Recognizing Millions
                  of Wikipedia Entities},
  booktitle    = {{IEEE/CVF} International Conference on Computer Vision, {ICCV} 2023,
                  Paris, France, October 1-6, 2023},
  pages        = {12031--12041},
  publisher    = {{IEEE}},
  year         = {2023},
  url          = {https://doi.org/10.1109/ICCV51070.2023.01108},
  doi          = {10.1109/ICCV51070.2023.01108},
  timestamp    = {Mon, 22 Jan 2024 17:21:08 +0100},
  biburl       = {https://dblp.org/rec/conf/iccv/HuLCKJLTC23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{llava,
  author       = {Haotian Liu and
                  Chunyuan Li and
                  Qingyang Wu and
                  Yong Jae Lee},
  editor       = {Alice Oh and
                  Tristan Naumann and
                  Amir Globerson and
                  Kate Saenko and
                  Moritz Hardt and
                  Sergey Levine},
  title        = {Visual Instruction Tuning},
  booktitle    = {Advances in Neural Information Processing Systems 36: Annual Conference
                  on Neural Information Processing Systems 2023, NeurIPS 2023, New Orleans,
                  LA, USA, December 10 - 16, 2023},
  year         = {2023},
  url          = {http://papers.nips.cc/paper\_files/paper/2023/hash/6dcf277ea32ce3288914faf369fe6de0-Abstract-Conference.html},
  timestamp    = {Fri, 01 Mar 2024 16:26:20 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/LiuLWL23a.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{blip2,
  author       = {Junnan Li and
                  Dongxu Li and
                  Silvio Savarese and
                  Steven C. H. Hoi},
  editor       = {Andreas Krause and
                  Emma Brunskill and
                  Kyunghyun Cho and
                  Barbara Engelhardt and
                  Sivan Sabato and
                  Jonathan Scarlett},
  title        = {{BLIP-2:} Bootstrapping Language-Image Pre-training with Frozen Image
                  Encoders and Large Language Models},
  booktitle    = {International Conference on Machine Learning, {ICML} 2023, 23-29 July
                  2023, Honolulu, Hawaii, {USA}},
  series       = {Proceedings of Machine Learning Research},
  volume       = {202},
  pages        = {19730--19742},
  publisher    = {{PMLR}},
  year         = {2023},
  url          = {https://proceedings.mlr.press/v202/li23q.html},
  timestamp    = {Mon, 04 Dec 2023 11:29:49 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/0008LSH23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{flamingo,
  author       = {Jean{-}Baptiste Alayrac and
                  Jeff Donahue and
                  Pauline Luc and
                  Antoine Miech and
                  Iain Barr and
                  Yana Hasson and
                  Karel Lenc and
                  Arthur Mensch and
                  Katherine Millican and
                  Malcolm Reynolds and
                  Roman Ring and
                  Eliza Rutherford and
                  Serkan Cabi and
                  Tengda Han and
                  Zhitao Gong and
                  Sina Samangooei and
                  Marianne Monteiro and
                  Jacob L. Menick and
                  Sebastian Borgeaud and
                  Andy Brock and
                  Aida Nematzadeh and
                  Sahand Sharifzadeh and
                  Mikolaj Binkowski and
                  Ricardo Barreira and
                  Oriol Vinyals and
                  Andrew Zisserman and
                  Kar{\'{e}}n Simonyan},
  editor       = {Sanmi Koyejo and
                  S. Mohamed and
                  A. Agarwal and
                  Danielle Belgrave and
                  K. Cho and
                  A. Oh},
  title        = {Flamingo: a Visual Language Model for Few-Shot Learning},
  booktitle    = {Advances in Neural Information Processing Systems 35: Annual Conference
                  on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans,
                  LA, USA, November 28 - December 9, 2022},
  year         = {2022},
  url          = {http://papers.nips.cc/paper\_files/paper/2022/hash/960a172bc7fbf0177ccccbb411a7d800-Abstract-Conference.html},
  timestamp    = {Mon, 08 Jan 2024 16:31:26 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/AlayracDLMBHLMM22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{instructblip,
  author       = {Wenliang Dai and
                  Junnan Li and
                  Dongxu Li and
                  Anthony Meng Huat Tiong and
                  Junqi Zhao and
                  Weisheng Wang and
                  Boyang Li and
                  Pascale Fung and
                  Steven C. H. Hoi},
  editor       = {Alice Oh and
                  Tristan Naumann and
                  Amir Globerson and
                  Kate Saenko and
                  Moritz Hardt and
                  Sergey Levine},
  title        = {InstructBLIP: Towards General-purpose Vision-Language Models with
                  Instruction Tuning},
  booktitle    = {Advances in Neural Information Processing Systems 36: Annual Conference
                  on Neural Information Processing Systems 2023, NeurIPS 2023, New Orleans,
                  LA, USA, December 10 - 16, 2023},
  year         = {2023},
  url          = {http://papers.nips.cc/paper\_files/paper/2023/hash/9a6a435e75419a836fe47ab6793623e6-Abstract-Conference.html},
  timestamp    = {Fri, 01 Mar 2024 16:26:20 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/Dai0LTZW0FH23.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{llava1.5,
  author       = {Haotian Liu and
                  Chunyuan Li and
                  Yuheng Li and
                  Yong Jae Lee},
  title        = {Improved Baselines with Visual Instruction Tuning},
  journal      = {CoRR},
  volume       = {abs/2310.03744},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2310.03744},
  doi          = {10.48550/ARXIV.2310.03744},
  eprinttype    = {arXiv},
  eprint       = {2310.03744},
  timestamp    = {Thu, 19 Oct 2023 13:12:52 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2310-03744.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{bai2023qwenvl,
      title={Qwen-VL: A Versatile Vision-Language Model for Understanding, Localization, Text Reading, and Beyond}, 
      author={Jinze Bai and Shuai Bai and Shusheng Yang and Shijie Wang and Sinan Tan and Peng Wang and Junyang Lin and Chang Zhou and Jingren Zhou},
      year={2023},
      eprint={2308.12966},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@inproceedings{realm,
  author       = {Kelvin Guu and
                  Kenton Lee and
                  Zora Tung and
                  Panupong Pasupat and
                  Ming{-}Wei Chang},
  title        = {Retrieval Augmented Language Model Pre-Training},
  booktitle    = {Proceedings of the 37th International Conference on Machine Learning,
                  {ICML} 2020, 13-18 July 2020, Virtual Event},
  series       = {Proceedings of Machine Learning Research},
  volume       = {119},
  pages        = {3929--3938},
  publisher    = {{PMLR}},
  year         = {2020},
  url          = {http://proceedings.mlr.press/v119/guu20a.html},
  timestamp    = {Tue, 15 Dec 2020 17:40:18 +0100},
  biburl       = {https://dblp.org/rec/conf/icml/GuuLTPC20.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{rag,
  author       = {Patrick S. H. Lewis and
                  Ethan Perez and
                  Aleksandra Piktus and
                  Fabio Petroni and
                  Vladimir Karpukhin and
                  Naman Goyal and
                  Heinrich K{\"{u}}ttler and
                  Mike Lewis and
                  Wen{-}tau Yih and
                  Tim Rockt{\"{a}}schel and
                  Sebastian Riedel and
                  Douwe Kiela},
  editor       = {Hugo Larochelle and
                  Marc'Aurelio Ranzato and
                  Raia Hadsell and
                  Maria{-}Florina Balcan and
                  Hsuan{-}Tien Lin},
  title        = {Retrieval-Augmented Generation for Knowledge-Intensive {NLP} Tasks},
  booktitle    = {Advances in Neural Information Processing Systems 33: Annual Conference
                  on Neural Information Processing Systems 2020, NeurIPS 2020, December
                  6-12, 2020, virtual},
  year         = {2020},
  url          = {https://proceedings.neurips.cc/paper/2020/hash/6b493230205f780e1bc26945df7481e5-Abstract.html},
  timestamp    = {Tue, 19 Jan 2021 15:57:07 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/LewisPPPKGKLYR020.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{robustrag,
  author       = {Ori Yoran and
                  Tomer Wolfson and
                  Ori Ram and
                  Jonathan Berant},
  title        = {Making Retrieval-Augmented Language Models Robust to Irrelevant Context},
  journal      = {CoRR},
  volume       = {abs/2310.01558},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2310.01558},
  doi          = {10.48550/ARXIV.2310.01558},
  eprinttype    = {arXiv},
  eprint       = {2310.01558},
  timestamp    = {Thu, 19 Oct 2023 13:12:52 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2310-01558.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{rome,
  author       = {Kevin Meng and
                  David Bau and
                  Alex Andonian and
                  Yonatan Belinkov},
  editor       = {Sanmi Koyejo and
                  S. Mohamed and
                  A. Agarwal and
                  Danielle Belgrave and
                  K. Cho and
                  A. Oh},
  title        = {Locating and Editing Factual Associations in {GPT}},
  booktitle    = {Advances in Neural Information Processing Systems 35: Annual Conference
                  on Neural Information Processing Systems 2022, NeurIPS 2022, New Orleans,
                  LA, USA, November 28 - December 9, 2022},
  year         = {2022},
  url          = {http://papers.nips.cc/paper\_files/paper/2022/hash/6f1d43d5a82a37e89b0665b33bf3a182-Abstract-Conference.html},
  timestamp    = {Mon, 08 Jan 2024 16:31:36 +0100},
  biburl       = {https://dblp.org/rec/conf/nips/MengBAB22.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{keyValueSukhbaatar2019,
  author       = {Sainbayar Sukhbaatar and
                  Edouard Grave and
                  Guillaume Lample and
                  Herv{\'{e}} J{\'{e}}gou and
                  Armand Joulin},
  title        = {Augmenting Self-attention with Persistent Memory},
  journal      = {CoRR},
  volume       = {abs/1907.01470},
  year         = {2019},
  url          = {http://arxiv.org/abs/1907.01470},
  eprinttype    = {arXiv},
  eprint       = {1907.01470},
  timestamp    = {Wed, 24 Jul 2019 16:34:28 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1907-01470.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{wei2023uniir,
  title={Uniir: Training and benchmarking universal multimodal information retrievers},
  author={Wei, Cong and Chen, Yang and Chen, Haonan and Hu, Hexiang and Zhang, Ge and Fu, Jie and Ritter, Alan and Chen, Wenhu},
  journal={arXiv preprint arXiv:2311.17136},
  year={2023}
}

@article{clip,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle={International conference on machine learning},
  pages={8748--8763},
  year={2021},
  organization={PMLR}
}

@inproceedings{vqa,
  title={Vqa: Visual question answering},
  author={Antol, Stanislaw and Agrawal, Aishwarya and Lu, Jiasen and Mitchell, Margaret and Batra, Dhruv and Zitnick, C Lawrence and Parikh, Devi},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={2425--2433},
  year={2015}
}

@InProceedings{okvqa,
author = {Kenneth Marino and Mohammad Rastegari and Ali Farhadi and Roozbeh Mottaghi},
title = {OK-VQA: A Visual Question Answering Benchmark Requiring External Knowledge},
booktitle = {Conference on Computer Vision and Pattern Recognition (CVPR)},
year = {2019},
}

@article{multiscript, 
title={MULTISCRIPT: Multimodal Script Learning for Supporting Open Domain Everyday Tasks}, 
volume={38}, 
url={https://ojs.aaai.org/index.php/AAAI/article/view/29854}, 
DOI={10.1609/aaai.v38i17.29854}, 
author={Qi, Jingyuan and Liu, Minqian and Shen, Ying and Xu, Zhiyang and Huang, Lifu}, 
year={2024}, month={Mar.}, 
pages={18888-18896} 
}
@article{faiss,
      title={The Faiss library},
      author={Matthijs Douze and Alexandr Guzhva and Chengqi Deng and Jeff Johnson and Gergely Szilvasy and Pierre-Emmanuel Mazaré and Maria Lomeli and Lucas Hosseini and Hervé Jégou},
      year={2024},
      eprint={2401.08281},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{wikiweb2m,
title={A Suite of Generative Tasks for Multi-Level Multimodal Webpage Understanding},
author={Andrea Burns and Krishna Srinivasan and Joshua Ainslie and Geoff Brown and Bryan A. Plummer and Kate Saenko and Jianmo Ni and Mandy Guo},
booktitle={The 2023 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
year={2023},
url={https://openreview.net/forum?id=rwcLHjtUmn}
}

@inproceedings{wit,
author = {Srinivasan, Krishna and Raman, Karthik and Chen, Jiecao and Bendersky, Michael and Najork, Marc},
title = {WIT: Wikipedia-Based Image Text Dataset for Multimodal Multilingual Machine Learning},
year = {2021},
isbn = {9781450380379},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3404835.3463257},
doi = {10.1145/3404835.3463257},
booktitle = {Proceedings of the 44th International ACM SIGIR Conference on Research and Development in Information Retrieval},
pages = {2443–2449},
numpages = {7},
keywords = {dataset, multimodal, machine learning, wikipedia, multilingual, image-text retrieval, neural networks},
location = {Virtual Event, Canada},
series = {SIGIR '21}
}

@article{hnsw,
  title={Efficient and robust approximate nearest neighbor search using hierarchical navigable small world graphs},
  author={Malkov, Yu A and Yashunin, Dmitry A},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={42},
  number={4},
  pages={824--836},
  year={2018},
  publisher={IEEE}
}

@inproceedings{plotqa,
  title={Plotqa: Reasoning over scientific plots},
  author={Methani, Nitesh and Ganguly, Pritha and Khapra, Mitesh M and Kumar, Pratyush},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={1527--1536},
  year={2020}
}

@article{laion,
  title={Laion-5b: An open large-scale dataset for training next generation image-text models},
  author={Schuhmann, Christoph and Beaumont, Romain and Vencu, Richard and Gordon, Cade and Wightman, Ross and Cherti, Mehdi and Coombes, Theo and Katta, Aarush and Mullis, Clayton and Wortsman, Mitchell and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={25278--25294},
  year={2022}
}

@misc{llava1.6,
    title={LLaVA-NeXT: Improved reasoning, OCR, and world knowledge},
    url={https://llava-vl.github.io/blog/2024-01-30-llava-next/},
    author={Liu, Haotian and Li, Chunyuan and Li, Yuheng and Li, Bo and Zhang, Yuanhan and Shen, Sheng and Lee, Yong Jae},
    month={January},
    year={2024}
}

@inproceedings{pali,
title={Pa{LI}: A Jointly-Scaled Multilingual Language-Image Model},
author={Xi Chen and Xiao Wang and Soravit Changpinyo and AJ Piergiovanni and Piotr Padlewski and Daniel Salz and Sebastian Goodman and Adam Grycner and Basil Mustafa and Lucas Beyer and Alexander Kolesnikov and Joan Puigcerver and Nan Ding and Keran Rong and Hassan Akbari and Gaurav Mishra and Linting Xue and Ashish V Thapliyal and James Bradbury and Weicheng Kuo and Mojtaba Seyedhosseini and Chao Jia and Burcu Karagol Ayan and Carlos Riquelme Ruiz and Andreas Peter Steiner and Anelia Angelova and Xiaohua Zhai and Neil Houlsby and Radu Soricut},
booktitle={The Eleventh International Conference on Learning Representations },
year={2023},
url={https://openreview.net/forum?id=mWVoBz4W0u}
}

@article{palix,
  publtype={informal},
  author={Xi Chen and Josip Djolonga and Piotr Padlewski and Basil Mustafa and Soravit Changpinyo and Jialin Wu and Carlos Riquelme Ruiz and Sebastian Goodman and Xiao Wang and Yi Tay and Siamak Shakeri and Mostafa Dehghani and Daniel Salz and Mario Lucic and Michael Tschannen and Arsha Nagrani and Hexiang Hu and Mandar Joshi and Bo Pang and Ceslee Montgomery and Paulina Pietrzyk and Marvin Ritter and A. J. Piergiovanni and Matthias Minderer and Filip Pavetic and Austin Waters and Gang Li and Ibrahim Alabdulmohsin and Lucas Beyer and Julien Amelot and Kenton Lee and Andreas Peter Steiner and Yang Li and Daniel Keysers and Anurag Arnab and Yuanzhong Xu and Keran Rong and Alexander Kolesnikov and Mojtaba Seyedhosseini and Anelia Angelova and Xiaohua Zhai and Neil Houlsby and Radu Soricut},
  title={PaLI-X: On Scaling up a Multilingual Vision and Language Model},
  year={2023},
  cdate={1672531200000},
  journal={CoRR},
  volume={abs/2305.18565},
  url={https://doi.org/10.48550/arXiv.2305.18565},
}

@inproceedings{clip2clip,
  title={Open-domain visual entity recognition: Towards recognizing millions of wikipedia entities},
  author={Hu, Hexiang and Luan, Yi and Chen, Yang and Khandelwal, Urvashi and Joshi, Mandar and Lee, Kenton and Toutanova, Kristina and Chang, Ming-Wei},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={12065--12075},
  year={2023}
}

@inproceedings{coco,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part V 13},
  pages={740--755},
  year={2014},
  organization={Springer}
}

@article{sharegpt4v,
  publtype={informal},
  author={Lin Chen and Jinsong Li and Xiaoyi Dong and Pan Zhang and Conghui He and Jiaqi Wang and Feng Zhao and Dahua Lin},
  title={ShareGPT4V: Improving Large Multi-Modal Models with Better Captions},
  year={2023},
  cdate={1672531200000},
  journal={CoRR},
  volume={abs/2311.12793},
  url={https://doi.org/10.48550/arXiv.2311.12793}
}

@inproceedings{aokvqa,
  title={A-okvqa: A benchmark for visual question answering using world knowledge},
  author={Schwenk, Dustin and Khandelwal, Apoorv and Clark, Christopher and Marino, Kenneth and Mottaghi, Roozbeh},
  booktitle={European conference on computer vision},
  pages={146--162},
  year={2022},
  organization={Springer}
}

@inproceedings{refcoco,
    title = "{R}efer{I}t{G}ame: Referring to Objects in Photographs of Natural Scenes",
    author = "Kazemzadeh, Sahar  and
      Ordonez, Vicente  and
      Matten, Mark  and
      Berg, Tamara",
    editor = "Moschitti, Alessandro  and
      Pang, Bo  and
      Daelemans, Walter",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D14-1086",
    doi = "10.3115/v1/D14-1086",
    pages = "787--798",
}

@inproceedings{lu2016visual,
  title={Visual relationship detection with language priors},
  author={Lu, Cewu and Krishna, Ranjay and Bernstein, Michael and Fei-Fei, Li},
  booktitle={Computer Vision--ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11--14, 2016, Proceedings, Part I 14},
  pages={852--869},
  year={2016},
  organization={Springer}
}

@misc{pascalvoc2007,
	author = "Everingham, M. and Van~Gool, L. and Williams, C. K. I. and Winn, J. and Zisserman, A.",
	title = "The {PASCAL} {V}isual {O}bject {C}lasses {C}hallenge 2007 {(VOC2007)} {R}esults",
	howpublished = "http://www.pascal-network.org/challenges/VOC/voc2007/workshop/index.html"}

@inproceedings{
vit,
title={An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
author={Alexey Dosovitskiy and Lucas Beyer and Alexander Kolesnikov and Dirk Weissenborn and Xiaohua Zhai and Thomas Unterthiner and Mostafa Dehghani and Matthias Minderer and Georg Heigold and Sylvain Gelly and Jakob Uszkoreit and Neil Houlsby},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=YicbFdNTTy}
}

@inproceedings{chen2024internvl,
  title={Internvl: Scaling up vision foundation models and aligning for generic visual-linguistic tasks},
  author={Chen, Zhe and Wu, Jiannan and Wang, Wenhai and Su, Weijie and Chen, Guo and Xing, Sen and Zhong, Muyan and Zhang, Qinglong and Zhu, Xizhou and Lu, Lewei and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={24185--24198},
  year={2024}
}

@article{llama2,
  title={Llama 2: Open foundation and fine-tuned chat models},
  author={Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert, Peter and Almahairi, Amjad and Babaei, Yasmine and Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal and Bhosale, Shruti and others},
  journal={arXiv preprint arXiv:2307.09288},
  year={2023}
}

@article{falcon,
  publtype={informal},
  author={Ebtesam Almazrouei and Hamza Alobeidli and Abdulaziz Alshamsi and Alessandro Cappelli and Ruxandra Cojocaru and Mérouane Debbah and Étienne Goffinet and Daniel Hesslow and Julien Launay and Quentin Malartic and Daniele Mazzotta and Badreddine Noune and Baptiste Pannier and Guilherme Penedo},
  title={The Falcon Series of Open Language Models},
  year={2023},
  cdate={1672531200000},
  journal={CoRR},
  volume={abs/2311.16867},
  url={https://doi.org/10.48550/arXiv.2311.16867}
}
